Knowledge-to-SQL: Enhancing SQL Generation with Data Expert LLM

Generating accurate SQL queries for user questions (text-to-SQL) has been a long-standing challenge since it requires a deep understanding of both the user's question and the corresponding database schema in order to retrieve the desired content accurately. Existing methods rely on the comprehensive capability of large language models (LLMs) to generate the SQL. However, some necessary knowledge is not explicitly included in the database schema and user question or has been learned by LLMs. Thus, the generated SQL of the knowledge-insufficient questions may be inaccurate, negatively influencing the text-to-SQL models' performance and robustness. To address this challenge, we propose the Knowledge-to-SQL framework, which employs tailored Data Expert LLM (DELLM) to provide helpful knowledge for all text-to-SQL models. Specifically, we introduce the detailed implementation of DELLM regarding table reading and the basic fine-tuning process. We further propose a Preference Learning via Database Feedback (PLDBF) strategy, refining the DELLM to generate more helpful knowledge for LLMs. Extensive experiments verify that DELLM can enhance the state-of-the-art approaches for text-to-SQL tasks. The corresponding code of DELLM is released for further research.

==> introv1.tex <==
% 第一段中最后一定要落在一个点：拥有对数据库的解释知识是至关重要的。
% Generate SQL according to user queries (text-to-SQL) is currently a leading real-world applications for Large Language models (LLMs). The most intuitive approach to input the user queries and database schema to LLMs and rely on LLMs to generate the SQL. However, in real-world application, user queries and database orginazation may contain some costumized or expertised knowledge. Under the such context, the intuitive approach may generate inaccurate or unexecuteable SQLs unless human expert input the necessary knowledge to the LLMs. Affected by this, it is awarding to develop a non-human arthitecture to automatedly generate the data expert knowledge in SQL generation to improve the performance and robustness of the text-to-SQL models.

Generating SQL based on user queries (Text-to-SQL) is currently one of the leading real-world applications for Large Language Models (LLMs). The most straightforward approach is to input the user queries and database schema into the LLMs and rely on them to generate the SQL~\cite{dou2022towards,liu2023comprehensive,pourreza2023dinsql}. However, in real-world applications, user queries and database organization may contain customized or specialized knowledge~\cite{yu2018Spider,li2023BIRD}. In such cases, the intuitive approach may result in inaccurate or un-executable SQL unless a human expert provides the necessary knowledge to the LLMs~\cite{li2023BIRD}. Given this challenge, it is valuable to develop a non-human architecture that can automatically generate the required data expert knowledge for SQL generation. This would significantly enhance the performance and robustness of text-to-SQL models.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figure/Intro.pdf}
    \caption{A sketch map illustrating the significance of incorporating expert knowledge in Text-to-SQL task.}
    \label{fig:intro}
\end{figure}

% 第二段要首先介绍recent和previous的方法
Existing models primarily focus on fully exploring the comprehensibility of Language Model. As the forerunner, T5-based methods~\cite{scholak2021picard,li2023graphix,rai2023improving} made an initial attempt to train a language model from scratch to generate SQL based on user queries and database schemas. Following the popularity of Language Models, particularly ChatGPT and GPT4~\cite{openai2023gpt}, DIN-SQL~\cite{pourreza2023dinsql} utilizes GPT to decompose the process of SQL generation into several sub-tasks. It uses GPT to first accomplish these sub-tasks and then aggregates the results to generate the SQL. Similarly, DAIL-SQL~\cite{gao2023text} refers to SQLs from similar queries to accomplish the generation of the required SQL. Most recently, MAC-SQL~\cite{wang2023mac} assigns different roles to three GPT4 agents, specifically Selector, Inspector, and Refiner, and uses these agents to contribute to the SQL generation process.

% However 他们缺少knowledge，标一下百分比，有多少的问题需要KNowledge才能回答正确
% However, existing models paying their main effort on design more complicated SQL generation structure to increase the SQL generation performance. However, there is a lack of emphsis on the necessarity of the data expert knowledge. As shown in the left of~\autoref{fig:intro}, without data expert solely rely on user's query and database schema cannot generate accurate condition. More seriously, the ``y.Date like '2012-08-\%''' may cause the SQL return blank data. On the contrary, on the right of~\autoref{fig:intro}, after given accurate data expert knowledge, the LLMs can rectify the condiction and generate the accurate SQL. 

However, existing models mainly focus on designing more complex SQL generation structures in order to improve SQL generation performance. However, there is a lack of emphasis on the necessity of data expert knowledge~\cite{li2023BIRD}. As depicted on the left of Figure~\ref{fig:intro}, relying solely on the user's query and the database schema without the data expert knowledge may generate inaccurate conditions. For example, the incorrect condition ``y.Date like "2012-08-\%"'' could potentially result in the SQL returning empty data. In contrast, on the right of Figure~\ref{fig:intro}, when provided with accurate data expert knowledge, the LLMs are able to rectify the condition and generate the valid SQL.


Nevertheless, generating expert knowledge from data faces the following challenges: 
\textbf{1. Query \& Database Specialization}: The generated expert knowledge should be specialized for the given query and database. It is challenging for the knowledge generator to understand the query and database and provide suitable knowledge. 
\textbf{2. Table Content Awareness}~\cite{cheng2023binding}: The expert should be able to read the content of the table in order to determine whether it is necessary to provide detailed content examples in the knowledge. 
\textbf{3. Performance Enhancement}~\cite{li2023BIRD}: The generated knowledge should be helpful for the SQL generation models. It is challenging to ensure that the expert knowledge can contribute to more accurate SQL generation.

% By solving the above challenge, we provide a complete \textbf{Knowledge-to-SQL} pipeline of generating data expert knowledge to enhance the SQL generation of LLMs. Specifically, we propose the detailed design of \textbf{Data Expert LLM (DELLM)} including the table reading component, the knowledge-based fine-tuning. Moreover, we propose the \textit{\underline{R}einforcement \underline{L}earning via \underline{D}atabase \underline{F}eedback (RLDBF)} to further ensure the generated data expert knowledge can be helpful in LLM-based SQL generation. Specifically, RLDBF give the DELLM reward according to two tailored criteria: 1. Whether the generated knowledge help in retrieving the accurate data, and 2. whether the generated knowledge helps LLM generate more accurate SQL.
% In summary, our contribution can listed as follow:

By addressing the aforementioned challenge, we present a complete \textbf{Knowledge-to-SQL} pipeline for enhancing the SQL generation of LLMs. Specifically, we propose a detailed design for the \textbf{Data Expert Language Model (DELLM)}, which comprises of a table reading component and a knowledge-oriented fine-tuning mechanism. Furthermore, we introduce \textit{\underline{R}einforcement \underline{L}earning via \underline{D}atabase \underline{F}eedback (RLDBF)} to further improve the helpfulness of the generated data expert knowledge in LLM-based SQL generation~\cite{christiano2017rlhf}. Specifically, RLDBF provides rewards to DELLM based on two tailored criteria: 1) the extent to which the generated knowledge aids in retrieving more accurate data, and 2) the degree to which the generated knowledge assists LLM in producing more precise SQL queries.
In summary, our contributions can be listed as follows:
% \begin{itemize}
%     \item We discover the importance of database knowledge and propose a complete Knowledge-to-SQL pipeline to enhance the SQL generation.
%     \item We provide a specially designed Data Expert LLM (DELLM) while introducing tailored fine-tuning and RL-tuning training strategy.
%     \item We opensoure the training and evaluation code of DELLM, as well as providing the parameter weight for further research.
%     \item We verify the effecitiveness of our approach on Bird and Spider dataset in improve the performance of general text-to-SQL models.
% \end{itemize}
\begin{itemize}
    \item We highlight the significance of data expert knowledge and present a comprehensive Knowledge-to-SQL pipeline for improving SQL generation.
    \item We introduce a specially designed Data Expert Language Model (DELLM), along with customized structure, fine-tuning technique, and RL-tuning training strategies.
    \item We release the training and evaluation code of DELLM as open source, and provide parameter weights for future research.
    \item We validate the effectiveness of our approach on the Bird and Spider datasets, demonstrating that DELLM can generally enhance the performance of common text-to-SQL models.
\end{itemize}
